SunDown: Model-driven Per-Panel Solar Anomaly Detection for Residential Arrays

There has been significant growth in both utility-scale and residential-scale solar installations in recent years, driven by rapid technology improvements and falling prices. Unlike utility-scale solar farms that are professionally managed and maintained, smaller residential-scale installations often lack sensing and instrumentation for performance monitoring and fault detection. As a result, faults may go undetected for long periods of time, resulting in generation and revenue losses for the homeowner. In this paper, we present SunDown, a sensorless approach designed to detect per-panel faults in residential solar arrays. SunDown does not require any new sensors for its fault detection and instead uses a model-driven approach that leverages correlations between the power produced by adjacent panels to detect deviations from expected behavior. SunDown can handle concurrent faults in multiple panels and perform anomaly classification to determine probable causes. Using two years of solar generation data from a real home and a manually generated dataset of multiple solar faults, we show that our approach has a MAPE of 2.98\% when predicting per-panel output. Our results also show that SunDown is able to detect and classify faults, including from snow cover, leaves and debris, and electrical failures with 99.13% accuracy, and can detect multiple concurrent faults with 97.2% accuracy.

==> algorithm_dataset.tex <==
\section{DATASET \& ALGORITHM}
\label{sec:data_algo}


\subsection{Dataset}
\label{sec:data_algo:data}

The per panel level dataset is obtained from a residential house located in Western Massachusetts, USA, where 31 panels are mounted side by side at four different roof planes. Each of those panels has 320W-capacity and equips with a microinverter. The entire system is setup since September 10, 2017, and the dataset is collected between September 13, 2017 to February 11, 2020 with average time interval of 5 minutes. Raw dataset contains power, DC voltage, DC current, AC voltage, AC frequency, and in-device temperature for each panel. The clean dataset combines the power output for all panels in time sequence and collaborates weather data from DarkSky API. The entire data is then separated into west roof, east roof, lower roof, and main roof sub-dataset based on the roof plane's section and facing direction.

The capacity level, correlation and system's condition have been carefully labeled based on daily power output from all panels in each sub-dataset. The capacity level is the ratio of maximum power output on that day with respect of maximum capacity of the panel, which is 320W. The correlation label shows how strong the power output of all panels correlate with each other. It can be also measured by calculating the Pearson correlation coefficient, which is used as one of the feature in anomaly detection. The condition label indicates the possible reasons for causing less correlated power output. The strong correlated data is labeled as normal, moderate correlated data is labeled as either partial shaded or object covered, and low correlated data is labeled as low power issue, production issue, and unknown issue. The relationship between each label is shown in table \ref{dataset_label}.

\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        Power Level & Correlation & Condition\\
        \hline
        High & Strong & Normal\\
        \hline
        High & Moderate & Partial Shaded\\
        \hline
        High & Moderate & Object Cover\\
        \hline
        Low & Low & Low Power Defect\\
        \hline
        Low & Low & Production Issue\\
        \hline
        High & Low & Unknown Issue\\
        \hline
    \end{tabular}
    \caption{Dataset Label}
    \label{dataset_label}
\end{table}



% \begin{figure*}
%       \centering
% \begin{minipage}{0.3\linewidth}
% %\centering  % redundant
% \includegraphics[width=\textwidth]{figures/normal_data_plot.jpg}
% \caption{Normal Label}
% \label{strong_corr}
% \end{minipage}%
% \hfill% not: "\hspace{0.5cm}"
% \begin{minipage}{0.3\linewidth}
% %\centering  % redundant
% \includegraphics[width=\textwidth]{figures/shaded_data_plot.jpg}
% \caption{Partial Shaded Label}
% \label{moderate_corr}
% \end{minipage}%
% \hfill% not: "\hspace{0.5cm}"
% \begin{minipage}{0.3\linewidth}
% %\centering  % redundant
% \includegraphics[width=\textwidth]{figures/snow_data_plot.jpg}
% \caption{Object Cover Label}
% \label{low_corr}
% \end{minipage}
% \end{figure*}

% \begin{figure*}
%       \centering
% \begin{minipage}{0.3\linewidth}
% %\centering  % redundant
% \includegraphics[width=\textwidth]{figures/syn_open.jpg}
% \caption{Synthetic Open Circuit}
% \label{syn_open}
% \end{minipage}%
% \hfill% not: "\hspace{0.5cm}"
% \begin{minipage}{0.3\linewidth}
% %\centering  % redundant
% \includegraphics[width=\textwidth]{figures/syn_cover.jpg}
% \caption{Synthetic Object Covering}
% \label{syn_cover}
% \end{minipage}%
% \hfill% not: "\hspace{0.5cm}"
% \begin{minipage}{0.3\linewidth}
% %\centering  % redundant
% \includegraphics[width=\textwidth]{figures/syn_multi.jpg}
% \caption{Synthetic Multiple Faults}
% \label{syn_multi}
% \end{minipage}
% \end{figure*}




% talk about the home
% talk about the different sets of panels (add an image of rooftop)
% talk about the solar panels
% age of the system

% \subsection{Algorithm}
% \label{sec:data_algo:algo}



% \subsubsection{System Level}
% \label{sec:data_algo:algo:system}

% \subsubsection{Panel Level}
% \label{sec:data_algo:algo:panel}
